UniRec: Unified Multimodal Encoding for LLM-Based Recommendations

Large language models have recently shown promise for multimodal recommendation, particularly with text and image inputs. Yet real-world recommendation signals extend far beyond these modalities. To reflect this, we formalize recommendation features into four modalities: text, images, categorical features, and numerical attributes, and highlight the unique challenges this heterogeneity poses for LLMs in understanding multimodal information. In particular, these challenges arise not only across modalities but also within them, as attributes such as price, rating, and time may all be numeric yet carry distinct semantic meanings. Beyond this intra-modality ambiguity, another major challenge is the nested structure of recommendation signals, where user histories are sequences of items, each associated with multiple attributes. To address these challenges, we propose UniRec, a unified multimodal encoder for LLM-based recommendation. UniRec first employs modality-specific encoders to produce consistent embeddings across heterogeneous signals. It then adopts a triplet representation, comprising attribute name, type, and value, to separate schema from raw inputs and preserve semantic distinctions. Finally, a hierarchical Q-Former models the nested structure of user interactions while maintaining their layered organization. Across multiple real-world benchmarks, UniRec outperforms state-of-the-art multimodal and LLM-based recommenders by up to 15%, and extensive ablation studies further validate the contributions of each component.

==> header.tex <==
% \documentclass[11pt]{article}

% \usepackage[preprint]{acl}
% % \usepackage[final]{acl}

% % Standard package includes
% \usepackage{times}
% \usepackage{latexsym}
% \usepackage{booktabs}
% \usepackage[T1]{fontenc}
% \usepackage[utf8]{inputenc}
% \usepackage{microtype}
% \usepackage{inconsolata}
% \usepackage{graphicx}


% % Recommended, but optional, packages for figures and better typesetting:
% \usepackage{microtype}
% \usepackage{graphicx}
% \usepackage{subfigure}
% \usepackage{booktabs} % for professional tables

% \usepackage{xcolor}
% \usepackage{xspace}
% \usepackage{tcolorbox}

% \definecolor{lightBlue}{rgb}{0.78, 0.85, 1.0}
% \definecolor{lightRed}{rgb}{1.0, 0.85, 0.85}
% \newtcbox{\bluebox}{on line, box align=base, colback=lightBlue,colframe=white,size=fbox,arc=3pt, before upper=\strut, top=-2pt, bottom=-4pt, left=-2pt, right=-2pt, boxrule=0pt}
% \newtcbox{\redbox}{on line, box align=base, colback=lightRed,colframe=white,size=fbox,arc=3pt, before upper=\strut, top=-2pt, bottom=-4pt, left=-2pt, right=-2pt, boxrule=0pt}
% \newcommand{\uarr}{$\uparrow$}
% \newcommand{\darr}{$\downarrow$}

% \usepackage{hyperref}
% \usepackage{multicol}
% \usepackage{multirow}
% \newcommand{\theHalgorithm}{\arabic{algorithm}}

% % For theorems and such
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{mathtools}
% \usepackage{amsthm}

% % if you use cleveref..
% \usepackage[capitalize,noabbrev]{cleveref}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % THEOREMS
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \theoremstyle{plain}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \theoremstyle{definition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{assumption}[theorem]{Assumption}
% \theoremstyle{remark}
% \newtheorem{remark}[theorem]{Remark}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % color
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \usepackage{colortbl}
% \usepackage{pgf} % for calculating the values for gradient
% \usepackage{xcolor} % enables the use of cellcolor
% \usepackage{graphicx}
% \usepackage{booktabs} % for better table formatting (optional)

% \definecolor{lightOliveGreen}{rgb}{0.75, 0.85, 0.65} % Light Olive Green (adjust as necessary)
% \definecolor{lightTomatoRed}{rgb}{1.0, 0.7, 0.6}     % Light Tomato Red (adjust as necessary)

% \newtcbox{\greenbox}{on line, box align=base, colback=lightOliveGreen, colframe=white, size=fbox, arc=3pt, before upper=\strut, top=-2pt, bottom=-4pt, left=-2pt, right=-2pt, boxrule=0pt}
% \newtcbox{\tomatobox}{on line, box align=base, colback=lightTomatoRed, colframe=white, size=fbox, arc=3pt, before upper=\strut, top=-2pt, bottom=-4pt, left=-2pt, right=-2pt, boxrule=0pt}





% % Color set related to your provided highlight.sty
% \definecolor{high}{HTML}{6B8E23}  % The color for increases (Olive Green)
% \definecolor{lowgreen}{HTML}{F0F8E7}  % A very light green for the lower end of the gradient
% \definecolor{redhigh}{HTML}{FF6347} % The color for decreases (Red, Tomato)
% \definecolor{lowred}{HTML}{FFE6E6}  % A very light red for the lower end of the gradient
% \newcommand{\opacity}{50}         % Opacity set to 50 (higher opacity, but you can reduce further if needed)

% % Gradient function for increases (Olive Green)
% \newcommand*{\minvaldiffa}{0}% define the minimum value on your data set
% \newcommand*{\maxvaldiffa}{50}% define the maximum value in your data set!
% \newcommand{\gcb}[1]{
%     \pgfmathparse{min(#1,\maxvaldiffa)}%
%     \xdef\clipval{\pgfmathresult}%
%     \pgfmathparse{max(\clipval,\minvaldiffa)}%
%     \xdef\clipval{\pgfmathresult}%
%     \pgfmathparse{int(round(100*(\clipval/(\maxvaldiffa-\minvaldiffa))-(\minvaldiffa*(100/(\maxvaldiffa-\minvaldiffa)))))}%
%     \xdef\tempa{\pgfmathresult}%
%     \cellcolor{high!\tempa!lowgreen!\opacity}%
%     $#1$%
% }

% % Gradient function for decreases (Red)
% \newcommand*{\minvaldiffb}{0}% define the minimum value on your data set
% \newcommand*{\maxvaldiffb}{50}% define the maximum value in your data set!
% \newcommand{\gca}[1]{
%     \pgfmathparse{min(#1,\maxvaldiffb)}%
%     \xdef\clipval{\pgfmathresult}%
%     \pgfmathparse{max(\clipval,\minvaldiffb)}%
%     \xdef\clipval{\pgfmathresult}%
%     \pgfmathparse{int(round(100*(\clipval/(\maxvaldiffb-\minvaldiffb))-(\minvaldiffb*(100/(\maxvaldiffb-\minvaldiffb)))))}%
%     \xdef\tempa{\pgfmathresult}%
%     \cellcolor{redhigh!\tempa!lowred!\opacity}%
%     $#1$%
% }


% \title{In-Context Learning May Not Elicit Trustworthy Reasoning: A-Not-B Errors in Pretrained Language Models}

% \author{%
%     Pengrui Han\thanks{Equal contribution.}\thanks{Work done as intern.}$^{\,1,3}$, Peiyang Song\footnotemark[1]$^{\,2}$, Haofei Yu$^{\,3}$, Jiaxuan You$^{\,3}$ \\
%     $^1$Carleton College, ~$^2$California Institute of Technology\\
%     $^3$University of Illinois Urbana-Champaign\\
%     \texttt{barryhan@carleton.edu}, \texttt{psong@caltech.edu} \\
% }

